An accelerated frequency-independent solver for oscillatory differential equations

Oscillatory second order linear ordinary differential equations arise in many scientific calculations. Because the running times of standard solvers increase linearly with frequency when they are applied to such problems, a variety of specialized methods, most of them quite complicated, have been proposed. Here, we point out that one of the simplest approaches not only works, but yields a scheme for solving oscillatory second order linear ordinary differential equations which is significantly faster than current state-of-the-art techniques. Our method, which operates by constructing a slowly varying phase function representing a basis of solutions of the differential equation, runs in time independent of the frequency and can be applied to second order equations whose solutions are oscillatory in some regions and slowly varying in others. In the high-frequency regime, our algorithm discretizes the nonlinear Riccati equation satisfied by the derivative of the phase function via a Chebyshev spectral collocation method and applies the Newton-Kantorovich method to the resulting system of nonlinear algebraic equations. We prove that the iterates converge quadratically to a nonoscillatory solution of the Riccati equation. The quadratic convergence of the Newton-Kantorovich method and the simple form of the linearized equations ensure that this procedure is extremely efficient. Our algorithm then extends the slowly varying phase function calculated in the high-frequency regime throughout the solution domain by solving a certain third order linear ordinary differential equation related to the Riccati equation. We describe the results of numerical experiments showing that our algorithm is orders of magnitude faster than existing schemes, including the modified Magnus method [18], the current state-of-the-art approach [7] and the recently introduced ARDC method [1].

==> experiments_magnus.tex <==
\begin{section}{Experiments}
\label{section:experiments}

In this section, we present the results of numerical experiments which were conducted to illustrate 
the properties of the method of this paper and to compare it with other solvers for oscillatory
differential equations. We implemented our algorithm in Fortran and compiled our code with  version 14.2.1 of the 
GNU Fortran compiler.    All experiments were performed on a desktop computer equipped
with an AMD 9950X processor and 64GB of RAM.  This processor  has 16 cores, but
only one core was utilized in our experiments.

In all of our experiments,  the value of the parameter $k$, which determines the order of the 
Chebyshev expansions used to represent phase functions, was taken to be $16$
and the parameter $\epsilon$  which controls the accuracy of the obtained phase functions
was set to $10^{-12}$.


In almost all of our experiments, we tested the accuracy of our method and those we compare it to 
by using it to calculate solutions to initial and boundary value problems for second
order equations. The experiment of   Section~\ref{section:experiments3},
in which the accuracy of the phase functions produced by our algorithm was measured
directly, is the sole exception.
Because the condition numbers of initial and boundary value problems for (\ref{introduction:ode}) 
grow with $\omega$, the accuracy of any numerical
method used to solve them is expected to deteriorate with increasing  frequency.    
In the case of our algorithm, the phase functions themselves are calculated to high precision, 
but the magnitudes of the phase functions  increase with frequency and accuracy is lost when 
the phase functions  are exponentiated.
One implication is that calculations which involve only the phase functions
and not the solutions of the scalar equation can be performed to high accuracy.
The article \cite{BremerZeros}, for example,  describes
a phase function method  for rapidly computing the zeros of solutions of second order linear ordinary
differential equations to extremely high accuracy.    

To account for the vagaries of modern computing environments, all reported times were obtained 
by averaging the cost of each calculation over 100 runs.  



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{Comparison with the Modified Magnus expansion method}
\label{section:experiments1}

In this first experiment, we compared the performance of the modified Magnus method of \cite{ModMagnus}, 
which is one of the most widely used methods for solving oscillatory differential equations,
with the algorithm of this paper.  The former is a step method
that combines an exponential integrator with  preconditioning via the solutions of a 
constant coefficient equation obtained by freezing the coefficient matrix of the oscillatory 
equation. We used a fourth order exponential integrator and 
equispaced step sizes in our implementation of the  modified Magnus method,
which was written in Fortran and closely follows the
description provided in \cite{ModMagnus} and \cite{Iserles2}.



For each $n=2^6, 2^7, 2^8, \ldots, 2^{20}$, we used both methods to evaluate the solution
%
\begin{equation}
L_n(x) = P_n(x) + i \frac{2}{\pi} Q_n(x)
\label{experiments:lnu}
\end{equation}
%
of Legendre's differential
%
\begin{equation}
(1-t^2) y''(t)  -2t y'(t) + n(n+1) y(t) = 0 
\label{experiments:legendre}
\end{equation}
%
at a collection of points on the interval $[0,0.9]$.  Because Equation~(\ref{experiments:lnu})
is not in the normal form (\ref{introduction:ode}), we actually applied the algorithm 
of this paper to the differential equation
%
\begin{equation}
y''(t) + \left(\frac{1}{(1-t^2)^2} + \frac{n(n+1)}{1-t^2} \right) y(t) = 0,
\label{experiments:legnormal}
\end{equation}
%
which has  $L_n(t)\sqrt{1-t^2}$ as a solution.
We choose to evaluate the Legendre function $L_n$ because its logarithmic derivative
is nonoscillatory.  We discuss this further  in Section~\ref{section:experiments3},
and it can be seen from the graph of the accuracy predicted by its
condition number of evaluation in Figure~\ref{experiments1:figure1}.


\begin{figure}[b!!!!!!!!!!!!!!!!!!!!]
\hfil
\includegraphics[width=.49\textwidth]{experiment1-times.pdf}
\hfil
\includegraphics[width=.49\textwidth]{experiment1-errs.pdf}
\hfil

\caption{The results of the experiment of Section~\ref{section:experiments1}
in which the modified Magnus method of \cite{ModMagnus} and the algorithm
of this paper were used to evaluate the Legendre function $L_n(t)$ defined in (\ref{experiments:lnu})
on the interval $[0,0.9]$.  
The plot on the left gives the time in seconds required by each method as a function
of the degree $n$ of the Legendre function, while the plot on the right
gives the maximum relative error observed in the course of evaluating  the Legendre function
using each method. The plot on the right  also shows the accuracy predicted by the 
condition number of evaluation of the Legendre function.
We give the results for the modified Magnus method when the step size $h$
was taken to be a constant multiple of  $n^{-1/2}$, and when it was taken to be a constant multiple of
 $n^{-3/4}$.  
}
\label{experiments1:figure1}
\end{figure}



For each value of $n$ considered,  we executed the modified Magnus method twice, once
with the step size $h$ taken to be a constant multiple of $n^{-1/2}$ 
and again with the step size taken to be the same constant multiple of $n^{-3/4}$.
The constant was set so as to ensure  $10^{-10}$ relative accuracy for 
the smallest value of $n$ considered.
We struggled to obtain higher accuracy with the modified Magnus
method at high frequencies because it becomes numerically unstable when the step size is 
extremely small. In the case of our algorithm, for each value of $n$ considered,
we evaluated $L_n$ at a collection of 1,000 equispaced points on the 
interval $[0,0.9]$ and recorded the largest relative error which was observed.
For the modified Magnus method, we recorded the largest
relative error which was observed at the steps taken by the solver.
Figure~\ref{experiments1:figure1} gives the results.  The plot on the left
shows   the time taken by each method as a function of $n$, while that on the right 
gives the largest observed relative errors, again as a function of $n$.  
The plot on the right also shows the relative accuracy predicted by the condition 
number of evaluation of the function $L_n$.  
More explicitly, it displays a graph of 
%
\begin{equation}
\kappa(n) = \max_{j=1,\ldots,100} \epsilon_0 \left|\frac{t_j L_n'(t_j) }{L_n(t_j)}\right|,
\end{equation}
%
where $t_1,\ldots,t_{100}$ are the equispaced nodes on $[0,0.9]$ at which
we evaluated $L_n$ using the algorithm of this paper and 
 $\epsilon_0 \approx 2.220446049250313\times 10^{-16}$
is machine zero. 




From Figure~\ref{experiments1:figure1}, we see that the modified Magnus method
maintains roughly constant accuracy when the number of steps scales
as $n^{3/4}$, but loses accuracy when the step size scales only as $n^{1/2}$.
This is consistent with the theoretical estimates presented in \cite{ModMagnus}.
The method of this paper is several orders of magnitude faster than the modified
Magnus method, even at low frequencies, and it is more than 4 orders of magnitude
faster at the highest frequency considered.
%% We note that while the accuracy obtained by our algorithm is higher than the modified Magnus
%% method, except at very high frequencies, and it closely matches
%% the relative accuracy predicted by the condition number of evaluation
%% of $L_n$ at all frequencies.



\end{subsection}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{Comparison with two frequency-independent solvers}
\label{section:experiments2}

\begin{figure}[t!!!!!!!!!!!!!!!!!!!!]
\hfil
\includegraphics[width=.49\textwidth]{experiment2-times.pdf}
\hfil
\includegraphics[width=.49\textwidth]{experiment2-errs.pdf}
\hfil


\caption{The results of the experiment of Subsection~\ref{section:experiments2}
in which the method of this paper, the smooth deformation scheme of \cite{BremerPhase}
and  the ARDC method of \cite{ARDC} were used to evaluate the Legendre function
$L_n$ defined in (\ref{experiments:lnu})
on the interval $[0,0.999]$.
The plot on the left gives the time required by each algorithm as a function of the degree
$n$ of the Legendre function,
while the plot on the right shows the maximum relative error observed
when $L_n$ was evaluated
at $100$ equispaced points on the interval $[0,.999]$ using each approach.
The plot on the right also gives the maximum relative error 
predicted by the condition number of evaluation of this function.
}
\label{experiments2:figure1}
\end{figure}

In this experiment, we compared the algorithm of this paper with the ARDC
method of \cite{ARDC} and the frequency-independent solver \cite{BremerPhase}
previously developed by one of this paper's authors
by once again evaluating the solution $L_n$ of Legendre's differential
equation (\ref{experiments:legendre}).
%% by evaluating a solution of Legendre's differential
%% equation  of Legendre's differential
%% %
%% \begin{equation}
%% (1-t^2) y''(t)  -2t y'(t) + n(n+1) y(t) = 0.
%% \label{experiments:legendre}
%% \end{equation}
%
More explicitly, for each $n=2^6, 2^7, 2^8, \ldots, 2^{20}$, we used each
method to compute  $L_n$
%% %
%% \begin{equation}
%% L_n(x) = P_n(x) + i \frac{2}{\pi} Q_n(x)
%% \label{experiments:lnu}
%% \end{equation}
%
at $100$ equispaced nodes on $[0,0.999]$, including 
the points $0$ and $0.999$.
%% Because Equation~(\ref{experiments:legendre})
%% is not in the normal form (\ref{introduction:ode}), we actually applied the algorithm 
%% of this paper to the differential equation
%% %% %
%% %% \begin{equation}
%% %% y''(t) + \left(\frac{1}{(1-t^2)^2} + \frac{n(n+1)}{1-t^2} \right) y(t) = 0,
%% %% \label{experiments:legnormal}
%% %% \end{equation}
%% %
%% which has  $L_n(t)\sqrt{1-t^2}$ as a solution.
%% We choose $L_n$ because it is the solution of Legendre's equation
%% associated which corresponds with the nonoscillatory phase function;
%% this is discussed further  in Section~\ref{section:experiments3}.
We evaluated $L_n$ at a relatively small number of nodes 
because the method of \cite{ARDC} is a step scheme which
only returns the values of the solution at a sparse set of 
nodes sampled well below the Nyquist frequency.  This means that the solution
returned by the ARDC method  cannot be accurately interpolated at  arbitrary
points on the solution domain.  In order to evaluate it at 
the  $100$ equispaced nodes we considered, we had to specify them as inputs
to ARDC and doing so increased the cost of the algorithm.  Adding more points would
increase the cost further, and we regard $100$ points as  sufficient
to measure the accuracy of the solution.    Both the algorithm
of this paper and that of \cite{BremerPhase} allow for the solution
to be evaluated at any point on the solution domain.

Figure~\ref{experiments2:figure1} gives the results of this experiment.
The plot on the left gives the time required by each method
as a function of $n$, while that on the right
shows the maximum relative accuracy achieved by each method as a function of $n$, 
as well as the relative accuracy predicted by the condition number of evaluation of $L_n$.
We note that the three methods achieve very similar levels of accuracy
for large values of $n$, while the the ARDC method loses some accuracy
at small values of $n$.  ARDC is noticeably slower than \cite{BremerPhase}, and it
is several orders of magnitude slower than the method of this paper.

\end{subsection}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{Accuracy of the computed phase functions}
\label{section:experiments3}


In this experiment, we  measured the accuracy with which our 
method  computes phase functions.  For each $n=2^7,2^8,\ldots,2^{21}$, we 
used our algorithm   to construct the derivative of a nonoscillatory
trigonometric phase function for the  normal form (\ref{experiments:legnormal}) of
Legendre's differential equation on the interval $\left[0,1-10^{-7}\right]$.


\begin{figure}[t!!!!!!!!!!!!!!!!!!!!]
\hfil
\includegraphics[width=.49\textwidth]{experiment3-times.pdf}
\hfil
\includegraphics[width=.49\textwidth]{experiment3-errs.pdf}
\hfil

\caption{The results of the experiment of Subsection~\ref{section:experiments3}
in which the accuracy of the phase functions computed by our algorithm
was measured.  The plot on the left 
gives the time taken by our algorithm as a function of $n$.
The plot on the right gives the maximum relative accuracy
observe while evaluating the solution of Kummer's equation calculated by our algorithm
at 1,000 points in the interval $\left[0,1-10^{-7}\right]$.
}
\label{experiments3:figure1}
\end{figure}

There is an explicit expression for  the desired solution of Kummer's equation in this case.
Indeed, it can be shown using the formula
%
\begin{equation}
 \left(P_n(t)\right)^2 + \frac{4}{\pi^2} \left(Q_n(t)\right)^2
= \frac{4}{\pi^2} \int_1^\infty Q_n\left(t^2 + (1-t^2)s\right) \frac{ds}{\sqrt{s^2-1}},
\ \ \ -1 < t < 1,
\label{experiments3:legemod}
\end{equation}
%
which appears in \cite{durand75}, that the function
on the  left-hand side of (\ref{experiments3:legemod}) is absolutely monotone on $(0,1)$.
Since the functions
%
\begin{equation}
\sqrt{\frac{\pi}{2}} P_n(t)\sqrt{1-t^2}, \ \ \ \frac{2}{\pi}  Q_n(t)\sqrt{1-t^2}
\label{experiments3:pq}
\end{equation}
%
are a pair of solutions of (\ref{experiments:legnormal})
whose Wronskian is $1$ (see, for instance, Chapter~3 of \cite{HTFI}), the function
%
\begin{equation}
\alpha'(t) = \frac{1}{\left(1-t^2\right)\left(\frac{\pi}{2}P_n^2(t) + \frac{2}{\pi} Q_n^2(t) \right)}.
\label{experiments3:kummer}
\end{equation}
%
is the derivative of the desired nonoscillatory trigonometric phase function
for the normal form of Legendre's differential equation.


For each value of $n$ considered in this experiment,
we measured the accuracy of the  obtained solution of Kummer's equation
by comparing it with the reference solution (\ref{experiments3:kummer})
at  at 1,000 equispaced points on the interval $\left[0,1-10^{-7}\right]$.
Figure~\ref{experiments3:figure1} 
gives the largest observed relative accuracy as a function of $n$,
as well as the time required to construct the phase function.
We observe that the phase function is always computed with
relative accuracy which is greater than the requested
precision $1.0 \times 10^{-12}$.  

\end{subsection}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{Evaluation of Gegenbauer polynomials}
\label{section:experiments4}
In the experiment of this section, we used the scheme of this paper 
to evaluate the Gegenbauer polynomials $C_n^{\alpha}(t)$, which are 
solutions of the differential equation
%
\begin{equation}
(1-t^2) y''(t) - 2(\alpha+1) y(t) + n(n+2 \alpha)y(t) = 0.
\label{experiments4:ode}
\end{equation}
%
For each $n=2^6,2^7,2^8,\ldots,2^{20}$ and $\alpha=-0.499,0.25,1.00$,
we computed a phase function for the normal form
%
\begin{equation}
y''(t) + \left(
\frac{\alpha-\alpha^2+\frac{3}{4}}{(1-t^2)^2}
+
\frac{\left(n+\alpha-\frac{1}{2}\right)\left(n+\alpha+\frac{1}{2}\right)}{1-t^2}
\right) y(t) = 0
\end{equation}
%
of (\ref{experiments4:ode}) satisfied by $C_n^{\alpha}(t)\left(1-t^2\right)^{(2\alpha+1)/4}$
via the algorithm of this paper and used
it to evaluate $C_n^{\alpha}(x)$ at 1,000 equispaced points on the
interval $(0,0.999)$.  
We compared the obtained values to those computed using the well-known three-term recurrence
relation satisfied by the Gegenbauer polynomials.
The results are shown in Figure~\ref{experiments4:figure1}.  There, 
we give the largest observed absolute error as a function of $n$,
as well as the time required to construct each  phase function.
We measured absolute error in these experiments because $C_n^\alpha$ has zeros
on the interval $(0,1)$.  

\begin{figure}[b!!!!!!!!!!!!!!!!!!!!]
\hfil 
\includegraphics[width=.49\textwidth]{experiment4-times.pdf}
\hfil
\includegraphics[width=.49\textwidth]{experiment4-errs.pdf}
\hfil

\caption{The results of the experiment of Subsection~\ref{section:experiments4}
in which our algorithm was used to evaluate Gegenbauer polynomials
of orders $\alpha=-0.499,0.25,1.0$.
The plot on the left  gives the time required to construct each phase function.
The plot on the right gives the maximum absolute accuracy observed
while evaluating the Gegenbauer polynomials at 1,000 equispaced
points on the interval $[0,0.999]$.
}
\label{experiments4:figure1}
\end{figure}

\end{subsection}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{A boundary value problem}
\label{section:experiments5}

In this final experiment, 
%% we solved a boundary value problem
%% for an oscillatory differential equation whose coefficient
%% was somewhat more complicated than in previous examples.
for each $\omega=2^6,2^7,\ldots,2^{20}$, 
we constructed a phase function for the differential equation
%
\begin{equation}
%% \left\{
%% \begin{aligned}
y''(t) + 
\omega ^2 \left(\frac{3 t^2
   \omega ^2+t^2 \omega
   +1}{-\left(t^2+1\right)
   \omega +\omega ^2+1}+\frac{2
   e^{-t}}{t^2+\frac{1}{10}}\right)
y''(t) = 0,\ \ \ -1 < t < 1,\ \ \ 
%% \end{aligned}
%% \right.
\label{experiments:bvp}
\end{equation}
%
and used it to evaluate the solution $y$ which satisfied the boundary conditions
 $y(-1) = y(1) = 1$ at 1,000 equispaced points on $[-1,1]$.  We then
applied  a standard adaptive Chebyshev spectral method to these boundary value problems
in order to construct reference solutions.
Figure~\ref{experiments5:figure1} gives the results.  The times required by our algorithm
and by the standard solver are plotted as functions of the frequency $\omega$
on the left, while the maximum observed
absolute error is plotted as a function of $\omega$ on the right.


\begin{figure}[h!!!!!!!!!!!!!!!!!!!!]
\hfil 
\includegraphics[width=.49\textwidth]{experiment5-times.pdf}
\hfil
\includegraphics[width=.49\textwidth]{experiment5-errs.pdf}
\hfil

\caption{The results of the experiment of Subsection~\ref{section:experiments5}
in which our algorithm was applied to boundary value problem for
the differential equation (\ref{experiments:bvp})
and the accuracy of the resulting solution was tested using
a standard adaptive Chebyshev spectral solver.
The plot on the left  gives the time required to solve the problem
using each method as a function of the frequency $\omega$,
while the plot on the right gives the maximum 
absolute error observed while comparing the  solution obtained using our method
with the reference solution computed via the standard solver.
}

\label{experiments5:figure1}
\end{figure}


\end{subsection}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% \begin{subsection}{Evaluation of solutions deep in the nonoscillatory regime}
%% \end{subsection}


\end{section}


==> experiments_nomagnus.tex <==
\begin{section}{Experiments}
\label{section:experiments}

In this section, we present the results of numerical experiments which were conducted to illustrate 
the properties of the method of this paper and to compare it with other solvers for oscillatory
differential equations. We implemented our algorithm in Fortran and compiled our code with  version 14.2.1 of the 
GNU Fortran compiler.    All experiments were performed on a desktop computer equipped
with an AMD 9950X processor and 64GB of RAM.  This processor  has 16 cores, but
only one core was utilized in our experiments.

In all of our experiments,  the value of the parameter $k$, which determines the order of the 
Chebyshev expansions used to represent phase functions, was taken to be $16$
and the parameter $\epsilon$  which controls the accuracy of the obtained phase functions
was set to $10^{-12}$.


In almost all of our experiments, we tested the accuracy of our method and those we compare it to 
by using it to calculate solutions to initial and boundary value problems for second
order equations. The experiment of   Section~\ref{section:experiments3},
in which the accuracy of the phase functions produced by our algorithm was measured
directly, is the sole exception.
Because the condition numbers of initial and boundary value problems for (\ref{introduction:ode}) 
grow with $\omega$, the accuracy of any numerical
method used to solve them is expected to deteriorate with increasing  frequency.    
In the case of our algorithm, the phase functions themselves are calculated to high precision, 
but the magnitudes of the phase functions  increase with frequency and accuracy is lost when 
the phase functions  are exponentiated.
One implication is that calculations which involve only the phase functions
and not the solutions of the scalar equation can be performed to high accuracy.
The article \cite{BremerZeros}, for example,  describes
a phase function method  for rapidly computing the zeros of solutions of second order linear ordinary
differential equations to extremely high accuracy.    

To account for the vagaries of modern computing environments, all reported times were obtained 
by averaging the cost of each calculation over 100 runs.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{Comparison with the Modified Magnus expansion method}
\label{section:experiments1}

In this first experiment, we compared the performance of the modified Magnus method of \cite{ModMagnus}, 
which is one of the most widely used methods for solving oscillatory differential equations,
with the algorithm of this paper.  The former is a step method
that combines an exponential integrator with  preconditioning via the solutions of a 
constant coefficient equation obtained by freezing the coefficient matrix of the oscillatory 
equation. We used a fourth order exponential integrator and 
equispaced step sizes in our implementation of the  modified Magnus method,
which was written in Fortran and closely follows the
description provided in \cite{ModMagnus} and \cite{Iserles2}.

For each $n=2^6, 2^7, 2^8, \ldots, 2^{20}$, we used both methods to evaluate the solution
%
\begin{equation}
L_n(x) = P_n(x) + i \frac{2}{\pi} Q_n(x)
\label{experiments:lnu}
\end{equation}
%
of Legendre's differential
%
\begin{equation}
(1-t^2) y''(t)  -2t y'(t) + n(n+1) y(t) = 0 
\label{experiments:legendre}
\end{equation}
%
at a collection of points on the interval $[0,0.9]$.  Becasue Equation~(\ref{experiments:lnu})
is not in the normal form (\ref{introduction:ode}), we actually applied the algorithm 
of this paper to the differential equation
%
\begin{equation}
y''(t) + \left(\frac{1}{(1-t^2)^2} + \frac{n(n+1)}{1-t^2} \right) y(t) = 0,
\label{experiments:legnormal}
\end{equation}
%
which has  $L_n(t)\sqrt{1-t^2}$ as a solution.
We choose to evaluate the Legendre function $L_n$ because its logarithmic derivative
is nonoscillatory.  We discuss this further  in Section~\ref{section:experiments3},
and it can be seen from the graph of the accuracy predicted by its
condition number of evaluation in Figure~\ref{experiments1:figure1}.



\begin{figure}[b!!!!!!!!!!!!!!!!!!!!]
\hfil
\includegraphics[width=.49\textwidth]{experiment1-times.pdf}
\hfil
\includegraphics[width=.49\textwidth]{experiment1-errs.pdf}
\hfil

\caption{The results of the experiment of Section~\ref{section:experiments1}
in which the modified Magnus method of \cite{ModMagnus} and the algorithm
of this paper were used to evaluate the Legendre function $L_n(t)$ defined in (\ref{experiments:lnu})
on the interval $[0,0.9]$.  
The plot on the left gives the time in seconds required by each method as a function
of the degree $n$ of the Legendre function, while the plot on the right
gives the maximum relative error observed in the course of evaluating  the Legendre function
using each method. The plot on the right  also shows the accuracy predicted by the 
condition number of evaluation of the Legendre function.
We give the results for the modified Magnus method when the step size $h$
was taken to be a constant multiple of  $n^{-1/2}$, and when it was taken to be a constant multiple of
 $n^{-3/4}$.  
}
\label{experiments1:figure1}
\end{figure}


For each value of $n$ considered,  we executed the modified Magnus method twice, once
with the step size $h$ taken to be a constant multiple of $n^{-1/2}$ 
and again with the step size taken to be the same constant multiple of $n^{-3/4}$.
The constant was set so as to ensure  $10^{-10}$ relative accuracy for 
the smallest value of $n$ considered.
We struggled to obtain higher accuracy with the modified Magnus
method at high frequencies because it becomes numerically unstable when the step size is 
extremely small. In the case of our algorithm, for each value of $n$ considered,
we evaluated $L_n$ at a collection of $1,000$ equispaced points on the 
interval $[0,0.9]$ and recorded the largest relative error which was observed.
For the modified Magnus method, we recorded the largest
relative error which was observed at the steps taken by the solver.
Figure~\ref{experiments1:figure1} gives the results.  The plot on the left
shows   the time taken by each method as a function of $n$, while that on the right 
gives the largest observed relative errors, again as a function of $n$.  
The plot on the right also shows the relative accuracy predicted by the condition 
number of evaluation of the function $L_n$.  
More explicitly, it displays a graph of 
%
\begin{equation}
\kappa(n) = \max_{j=1,\ldots,100} \epsilon_0 \left|\frac{t_j L_n'(t_j) }{L_n(t_j)}\right|,
\end{equation}
%
where $t_1,\ldots,t_{100}$ are the equispaced nodes on $[0,0.9]$ at which
we evaluated $L_n$ using the algorithm of this paper and 
 $\epsilon_0 \approx 2.220446049250313\times 10^{-16}$
is machine zero. 




From Figure~\ref{experiments1:figure1}, we see that the modified Magnus method
maintains roughly constant accuracy when the number of steps scales
as $n^{3/4}$, but loses accuracy when the step size scales only as $n^{1/2}$.
This is consistent with the theoretical estimates presented in \cite{ModMagnus}.
The method of this paper is several orders of magnitude faster than the modified
Magnus method, even at low frequencies, and it is more than 4 orders of magnitude
faster at the highest frequency considered.
%% We note that while the accuracy obtained by our algorithm is higher than the modified Magnus
%% method, except at very high frequencies, and it closely matches
%% the relative accuracy predicted by the condition number of evaluation
%% of $L_n$ at all frequencies.


\end{subsection}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{Comparison with two frequency-independent solvers}
\label{section:experiments2}

\begin{figure}[t!!!!!!!!!!!!!!!!!!!!]
\hfil
\includegraphics[width=.49\textwidth]{experiment2-times.pdf}
\hfil
\includegraphics[width=.49\textwidth]{experiment2-errs.pdf}
\hfil


\caption{The results of the experiment of Subsection~\ref{section:experiments2}
in which the method of this paper, the smooth deformation scheme of \cite{BremerPhase}
and  the ARDC method of \cite{ARDC} were used to evaluate the Legende function
$L_n$ defined in (\ref{experiments:lnu})
on the interval $[0,0.999]$.
The plot on the left gives the time required by each algorithm as a function of the degree
$n$ of the Legendre function,
while the plot on the right shows the maximum relative error observed
when $L_n$ was evaluated
at $100$ equispaced points on the interval $[0,.999]$ using each approach.
The plot on the right also gives the maximum relative error 
predicted by the condition number of evaluation of this function.
}
\label{experiments2:figure1}
\end{figure}

In this experiment, we compared the algorithm of this paper with the ARDC
method of \cite{ARDC} and the frequency-independent solver \cite{BremerPhase}
previously developed by one of this paper's authors
by evaluating a solution of Legendre's differential
equation  of Legendre's differential
%
\begin{equation}
(1-t^2) y''(t)  -2t y'(t) + n(n+1) y(t) = 0.
\label{experiments:legendre}
\end{equation}
%
More explicitly, for each $n=2^6, 2^7, 2^8, \ldots, 2^{20}$, we used each
method to compute 
%
\begin{equation}
L_n(x) = P_n(x) + i \frac{2}{\pi} Q_n(x)
\label{experiments:lnu}
\end{equation}
%
at $100$ equispaced nodes on $[0,0.999]$, including 
the points $0$ and $0.999$.
Because Equation~(\ref{experiments:legendre})
is not in the normal form (\ref{introduction:ode}), we actually applied the algorithm 
of this paper to the differential equation
%
\begin{equation}
y''(t) + \left(\frac{1}{(1-t^2)^2} + \frac{n(n+1)}{1-t^2} \right) y(t) = 0,
\label{experiments:legnormal}
\end{equation}
%
which has  $L_n(t)\sqrt{1-t^2}$ as a solution.
We choose $L_n$ because it is the solution of Legendre's equation
associated which corresponds with the nonoscillatory phase function;
this is discussed further  in Section~\ref{section:experiments3}.
We evaluated $L_n$ at a relatively small number of nodes 
because the method of \cite{ARDC} is a step scheme which
only returns the values of the solution at a sparse set of 
nodes sampled well below the Nyquist frequency.  This means that the solution
returned by the ARDC method  cannot be accurately interpolated at  arbitrary
points on the solution domain.  In order to evaluate it at 
the  $100$ equispaced nodes we considered, we had to specify them as inputs
to ARDC and doing so increased the cost of the algorithm.  Adding more points would
increase the cost further, and we regard $100$ points as  sufficient
to measure the accuracy of the solution.    Both the algorithm
of this paper and that of \cite{BremerPhase} allow for the solution
to be evaluated at any point on the solution domain.

Figure~\ref{experiments2:figure1} gives the results of this experiment.
The plot on the left gives the time required by each method
as a function of $n$, while that on the right
shows the maximum relative accuracy achieved by each method as a function of $n$, 
as well as the relative accuracy predicted by the condition number of evaluation of $L_n$.
We note that the three methods achieve very similar levels of accuracy
for large values of $n$, while the the ARDC method loses some accuracy
at small values of $n$.  ARDC is noticably slower than \cite{BremerPhase}, and it
is several orders of magnitude slower than the method of this paper.

\end{subsection}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{Accuracy of the computed phase functions}
\label{section:experiments3}


In this experiment, we  measured the accuracy with which our 
method  computes phase functions.  For each $n=2^7,2^8,\ldots,2^{21}$, we 
used our algorithm   to construct the derivative of a nonoscillatory
trigonometric phase function for the  normal form (\ref{experiments:legnormal}) of
Legendre's differential equation on the interval $\left[0,1-10^{-7}\right]$.

There is an explicit expression for  the desired solution of Kummer's equation in this case.
Indeed, it can be shown using the formula
%
\begin{equation}
 \left(P_n(t)\right)^2 + \frac{4}{\pi^2} \left(Q_n(t)\right)^2
= \frac{4}{\pi^2} \int_1^\infty Q_n\left(t^2 + (1-t^2)s\right) \frac{ds}{\sqrt{s^2-1}},
\ \ \ -1 < t < 1,
\label{experiments3:legemod}
\end{equation}
%
which appears in \cite{durand75}, that the function
on the  left-hand side of (\ref{experiments3:legemod}) is absolutely monotone on $(0,1)$.
Since the functions
%
\begin{equation}
\sqrt{\frac{\pi}{2}} P_n(t)\sqrt{1-t^2}, \ \ \ \frac{2}{\pi}  Q_n(t)\sqrt{1-t^2}
\label{experiments3:pq}
\end{equation}
%
are a pair of solutions of (\ref{experiments:legnormal})
whose Wronskian is $1$ (see, for instance, Chapter~3 of \cite{HTFI}), the function
%
\begin{equation}
\alpha'(t) = \frac{1}{\left(1-t^2\right)\left(\frac{\pi}{2}P_n^2(t) + \frac{2}{\pi} Q_n^2(t) \right)}.
\label{experiments3:kummer}
\end{equation}
%
is the derivative of the desired nonoscillatory trigonometric phase function
for the normal form of Legendre's differential equation.


\begin{figure}[b!!!!!!!!!!!!!!!!!!!!]
\hfil
\includegraphics[width=.49\textwidth]{experiment3-times.pdf}
\hfil
\includegraphics[width=.49\textwidth]{experiment3-errs.pdf}
\hfil

\caption{The results of the experiment of Subsection~\ref{section:experiments3}
in which the accuracy of the phase functions computed by our algorithm
was measured.  The plot on the left 
gives the time taken by our algorithm as a function of $n$.
The plot on the right gives the maximum relative accuracy
observe while evaluating the solution of Kummer's equation calculated by our algorithm
at $1,000$ points in the interval $\left[0,1-10^{-7}\right]$.
}
\label{experiments3:figure1}
\end{figure}

For each value of $n$ considered in this experiment,
we measured the accuracy of the  obtained solution of Kummer's equation
by comparing it with the reference solution (\ref{experiments3:kummer})
at  at $1,000$ equispaced points on the interval $\left[0,1-10^{-7}\right]$.
Figure~\ref{experiments3:figure1} 
gives the largest observed relative accuracy as a function of $n$,
as well as the time required to construct the phase function.
We observe that the phase function is always computed with
relative accuracy which is greater than the requested
precision $1.0 \times 10^{-12}$.  

\end{subsection}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{Evaluation of Gegenbauer polynomials}
\label{section:experiments4}
In the experiment of this section, we used the scheme of this paper 
to evaluate the Gegenbauer polynomials $C_n^{\alpha}(t)$, which are 
solutions of the differential equation
%
\begin{equation}
(1-t^2) y''(t) - 2(\alpha+1) y(t) + n(n+2 \alpha)y(t) = 0.
\label{experiments4:ode}
\end{equation}
%
For each $n=2^6,2^7,2^8,\ldots,2^{20}$ and $\alpha=-0.499,0.25,1.00$,
we computed a phase function for the normal form
%
\begin{equation}
y''(t) + \left(
\frac{\alpha-\alpha^2+\frac{3}{4}}{(1-t^2)^2}
+
\frac{\left(n+\alpha-\frac{1}{2}\right)\left(n+\alpha+\frac{1}{2}\right)}{1-t^2}
\right) y(t) = 0
\end{equation}
%
of (\ref{experiments4:ode}) satisfied by $C_n^{\alpha}(t)\left(1-t^2\right)^{(2\alpha+1)/4}$
via the algorithm of this paper and used
it to evaluate $C_n^{\alpha}(x)$ at $1,000$ equispaced points on the
interval $(0,0.999)$.  We allowed our code to use up to $16$ threads of execution.
We compared the obtained values to those computed using the well-known three-term recurrence
relation satisfied by the Gegenbauer polynomials.
The results are shown in Figure~\ref{experiments4:figure1}.  There, 
we give the largest observed absolute error as a function of $n$,
as well as the time required to construct each  phase function.
We measured absolute error in these experiments because $C_n^\alpha$ has zeros
on the interval $(0,1)$.  

\begin{figure}[b!!!!!!!!!!!!!!!!!!!!]
\hfil 
\includegraphics[width=.49\textwidth]{experiment4-times.pdf}
\hfil
\includegraphics[width=.49\textwidth]{experiment4-errs.pdf}
\hfil

\caption{The results of the experiment of Subsection~\ref{section:experiments4}
in which our algorithm was used to evaluate Gegenbauer polynomials
of orders $\alpha=-0.499,0.25,1.0$.
The plot on the left  gives the time required to construct each phase function.
The plot on the right gives the maximum absolute accuracy observed
while evaluating the Gegenbauer polynomials at $1,000$ equispaced
points on the interval $[0,0.999]$.
}
\label{experiments4:figure1}
\end{figure}

\end{subsection}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{A boundary value problem}
\label{section:experiments5}

In this final experiment, 
%% we solved a boundary value problem
%% for an oscillatory differential equation whose coefficient
%% was somewhat more complicated than in previous examples.
for each $\omega=2^6,2^7,\ldots,2^{20}$, 
we constructed a phase function for the differential equation
%
\begin{equation}
%% \left\{
%% \begin{aligned}
y''(t) + 
\omega ^2 \left(\frac{3 t^2
   \omega ^2+t^2 \omega
   +1}{-\left(t^2+1\right)
   \omega +\omega ^2+1}+\frac{2
   e^{-t}}{t^2+\frac{1}{10}}\right)
y''(t) = 0,\ \ \ -1 < t < 1,\ \ \ 
%% \end{aligned}
%% \right.
\label{experiments:bvp}
\end{equation}
%
and used it to evaluate te solution $y$ which satisfied the boundary conditions
 $y(-1) = y(1) = 1$ at $1,000$ equispaced points on $[-1,1]$.  We then
applied  a standard adaptive Chebyshev spectral method to these boundary value problems
in order to construct reference solutions and check the accuracy of our algorithm.
Figure~\ref{experiments5:figure1} gives the results.  The times required by our algorithm
and by the standard solver are given as functions of the frequency $\omega$
in the plot appearing on the left, while the maximum observed
absolute error is plotted as a function of $\omega$ on the right.


\begin{figure}[h!!!!!!!!!!!!!!!!!!!!]
\hfil 
\includegraphics[width=.49\textwidth]{experiment5-times.pdf}
\hfil
\includegraphics[width=.49\textwidth]{experiment5-errs.pdf}
\hfil

\caption{The results of the experiment of Subsection~\ref{section:experiments5}
in which our algorithm was applied to boundary value problem for
the differential equation (\ref{experiments:bvp})
and the accuracy of the resulting solution was tested using
a standard adaptive Chebyshev spectral solver.
The plot on the left  gives the time required to solve the problem
using each method as a function of the frequency $\omega$,
while the plot on the right gives the maximum 
absolute error observed while comparing the  solution obtained using our method
with the reference solution computed via the standard solver.
}

\label{experiments5:figure1}
\end{figure}


\end{subsection}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% \begin{subsection}{Evaluation of solutions deep in the nonoscillatory regime}
%% \end{subsection}


\end{section}

